Fast-DetectGPT: Efficient Zero-Shot Detection of Machine-Generated Text via Conditional Probability Curvature

Large language models (LLMs) have shown the ability to produce fluent and cogent content, presenting both productivity opportunities and societal risks. To build trustworthy AI systems, it is imperative to distinguish between machine-generated and human-authored content. The leading zero-shot detector, DetectGPT, showcases commendable performance but is marred by its intensive computational costs. In this paper, we introduce the concept of conditional probability curvature to elucidate discrepancies in word choices between LLMs and humans within a given context. Utilizing this curvature as a foundational metric, we present **Fast-DetectGPT**, an optimized zero-shot detector, which substitutes DetectGPT's perturbation step with a more efficient sampling step. Our evaluations on various datasets, source models, and test conditions indicate that Fast-DetectGPT not only surpasses DetectGPT by a relative around 75% in both the white-box and black-box settings but also accelerates the detection process by a factor of 340, as detailed in Table 1. See \url{https://github.com/baoguangsheng/fast-detect-gpt} for code, data, and results.

==> figures/probability_curvature.tex <==

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/probability-curvature.pdf}
    \caption{From probability curvature to sample distribution. The \emph{left figure} indicates that the samples conditioned on machine-generated text tend to have lower log probability than the original text, while the samples conditioned on human-written text may have higher or lower log probabilities than the original text.  The \emph{right figure} maps the probability curvature to the real distribution of conditional samples, where machine-generated and human-written texts occupy different regions of sample discrepancy.}
    \label{fig:probability-curvature}
\end{figure}

==> tables/cross_results.tex <==
\begin{table}[H]
    \centering\small
    \begin{tabular}{ccccccccccccc}
        \toprule
        Source & \multicolumn{4}{c}{\textbf{DetectGPT} (Scoring Model)} & \multicolumn{4}{c}{\textbf{Fast-DetectGPT} (Scoring Model)}  & \multicolumn{4}{c}{\textbf{Fast-DetectGPT} (GPT-J/Scoring Model)} \\        
        Model & GPT-2 & GPT-Neo & GPT-J & Avg. & GPT-2 & GPT-Neo & GPT-J & Avg. & GPT-2 & GPT-Neo & GPT-J & Avg. \\
        \midrule
        GPT-2 & 0.99 & 0.85 & 0.60 & 0.81 & 0.9953 & 0.9433 & 0.8557 & \bf 0.9314 &  0.9974 & 0.9787 & 0.8557 & 0.9439 \\
        GPT-Neo & 0.83 & 0.97 & 0.64 & 0.81 & 0.8786 & 0.9940 & 0.8630 & \bf 0.9119 & 0.9601 & 0.9985& 0.8630 & 0.9405 \\
        GPT-J & 0.79 & 0.83 & 0.92 & 0.85 & 0.8388 & 0.9279 & 0.9863 & \bf 0.9177 & 0.9313 & 0.9617 & 0.9863 & 0.9598 \\
        Avg. & 0.87 & 0.88 & 0.72 & - & \bf 0.9042 & \bf 0.9551 & \bf 0.9017 & - & 0.9629 & 0.9797 & 0.9017 & - \\
        \bottomrule
    \end{tabular}
    \caption{Zero-shot detection. Fast-DetectGPT outperforms DetectGPT with a large margin on the black-box settings.}
    \label{tab:cross_results}
\end{table}

==> tables/supervised.tex <==
\begin{figure*}[t]
    \begin{minipage}{0.5\linewidth}
        \centering\scriptsize
        \begin{tabular}{@{}lcccc@{}}
            \toprule
            \bf Method & \bf PubMedQA & \bf XSum & \bf WritingP & \bf Avg. \\
            \midrule
            RoBERTa-base & 0.6370 & 0.8986 & 0.9282 & 0.8213 \\
            RoBERTa-large & 0.6894 & 0.9325 & 0.9113 & 0.8444 \\
            \midrule
            DetectGPT $\diamondsuit$ & \bf 0.84 & 0.84 & 0.87 & 0.85 \\
            \midrule
            DetectGPT & 0.6977 & 0.8455 & 0.7818 & 0.7750 \\
            % Fast-DetectGPT (GPT-2/GPT-2) & 0.6572 & 0.8579 & 0.9110 & 0.8087 \\
            % Fast-DetectGPT (OPT-2.7) & 0.6865 & 0.9226 & 0.9464 & 0.8518 \\
            % Fast-DetectGPT (Neo-2.7/Neo-2.7) & 0.6819 & 0.9337 & 0.9419 & 0.8525 \\
            % Fast-DetectGPT (NeoX) & 0.6416 & 0.9277 & 0.9562 & 0.8418 \\
            Fast-DetectGPT & 0.7595* & 0.9134 & 0.9534* & \bf 0.8754 \\
            Fast-DetectGPT & 0.7225 & \bf 0.9391 & 0.9492 & 0.8703* \\
            Fast-DetectGPT & 0.6667 & 0.9331* & \bf 0.9575 & 0.8524 \\        
            \bottomrule
        \end{tabular}
        \caption{Detection of GPT-3 generations, evaluated in AUROC. Fast-DetectGPT in black-box settings (using given models) significantly outperforms DetectGPT in while-box settings (using GPT-3) on XSum and WritingP. Fast-DetectGPT uses 6B GPT-J to generate samples and from 1.5B GPT-2 to 6B GPT-J to score samples, while DetectGPT uses 11B T5 to generate perturbations and GPT-3 service to score them.  $\diamondsuit$ -- we report the official scores here instead of rerunning the experiments after confirming the consistency of the scores on RoBERTa.}
        \label{tab:gpt3_results}
    \end{minipage}
    \hfill
    \begin{minipage}{0.46\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{figures/supervised_barchart.pdf}
        \caption{Detection of generations for in-distribution (upper row) and out-distribution (down row) of the supervised classifiers. Fast-DetectGPT and DetectGPT perform as well as or better than the supervised classifiers on in-distribution datasets but achieve much better detection accuracy on out-distribution datasets. Furthermore, Fast-DetectGPT outperforms DetectGPT on all the four datasets.}
        \label{fig:supervised-bartchart}
    \end{minipage}
\end{figure*}


==> tables/supervised_results.tex <==
\begin{table}[t]
    \centering\small
    \begin{tabular}{lcccc}
        \toprule
        \bf Method & XSum (GPT-2) & PubMedQA (PubMedGPT) & WMT16-en (mGPT) & WMT16-de (mGPT) \\
        \midrule
        RoBERTa-base & 0.9813 & 0.6041 & 0.8888 & 0.4179 \\
        RoBERTa-large & \bf 0.9986 & 0.7115 & 0.9432 & 0.5502 \\
        \midrule
        Likelihood & 0.9006 & 0.7656 & 0.8378 & 0.7937 \\
        Rank & 0.8029 & 0.6637 & 0.7946 & 0.8369 \\
        LogRank & 0.9288 & 0.7703 & 0.8627 & 0.86 \\
        Entropy & 0.5515 & 0.4464 & 0.5091 & 0.6042 \\
        DetectGPT & 0.9885 & 0.8177 & 0.9585 & 0.9635 \\
        Fast-DetectGPT & 0.9934 & \bf 0.8479 & \bf 0.9840 & \bf 0.9973 \\
        \bottomrule
    \end{tabular}
    \caption{Compare with Supervised Detectors, evaluated in AUROC.}
    \label{tab:supervised_results}
\end{table}

==> tables/temperature_results.tex <==
\begin{table}[t]
    \centering\scriptsize
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\bf Dataset} & \multirow{2}{*}{\bf Method} & \multicolumn{6}{c}{\bf Source Model} \\
         &  & GPT-2 & OPT-2.7 & Neo-2.7 & GPT-J & NeoX & \bf Avg. \\    
        \midrule
        \multirow{10}{*}{XSum} 
        & Likelihood & 0.9781 & 0.9820 & 0.9862 & 0.9679 & 0.9511 & 0.9730 \\
        & Entropy & 0.5022 & 0.4289 & 0.4669 & 0.4837 & 0.5453 & 0.4854 \\
        & LogRank & 0.9883 & 0.9885 & 0.9939 & 0.9817 & 0.9694 & 0.9844 \\
        & LRR & 0.9889 & 0.9823 & 0.9910 & 0.9806 & 0.9702 & 0.9826 \\
        & NPR & 0.9955 & 0.9916 & 0.9976 & 0.9853 & 0.9760 & 0.9892 \\
        \cdashline{2-8}
        & DetectGPT & 0.9928 & 0.9856 & 0.9953 & 0.9790 & 0.9622 & 0.9830 \\
        & Fast-DetectGPT & 0.9999 & 0.9999 & 0.9997 & 0.9999 & 0.9997 & 0.9998 \\
        & \it (Diff) & \it 0.0071 & \it 0.0143 & \it 0.0044 & \it 0.0209 & \it 0.0376 & \it 0.0168 \\
        \cdashline{2-8}
        & DetectGPT & 0.9722 & 0.9635 & 0.9953 & 0.9627 & 0.9646 & 0.9717 \\
        & Fast-DetectGPT & 0.9978 & 0.9990 & 0.9999 & 0.9991 & 0.9980 & 0.9988 \\
        & \it (Diff) & \it 0.0256 & \it 0.0355 & \it 0.0046 & \it 0.0364 & \it 0.0333 & \it 0.0271 \\
        \midrule
        \multirow{10}{*}{SQuAD}
        & Likelihood & 0.9906 & 0.9870 & 0.9792 & 0.9572 & 0.9094 & 0.9647 \\
        & Entropy & 0.5132 & 0.4508 & 0.4924 & 0.4882 & 0.5263 & 0.4942 \\
        & LogRank & 0.9972 & 0.9959 & 0.9940 & 0.9798 & 0.9434 & 0.9821 \\
        & LRR & 0.9991 & 0.9973 & 0.9992 & 0.9911 & 0.9748 & 0.9923 \\
        & NPR & 0.9988 & 0.9963 & 0.9931 & 0.9684 & 0.8981 & 0.9710 \\
        \cdashline{2-8}
        & DetectGPT & 0.9959 & 0.9819 & 0.9778 & 0.9123 & 0.8132 & 0.9362 \\
        & Fast-DetectGPT & 1.0000 & 1.0000 & 1.0000 & 0.9994 & 0.9986 & 0.9996 \\
        & \it (Diff) & \it 0.0041 & \it 0.0180 & \it 0.0222 & \it 0.0871 & \it 0.1854 & \it 0.0634 \\
        \cdashline{2-8}
        & DetectGPT & 0.8936 & 0.8620 & 0.9778 & 0.8897 & 0.8898 & 0.9026 \\
        & Fast-DetectGPT & 1.0000 & 0.9999 & 1.0000 & 0.9984 & 0.9961 & 0.9989 \\
        & \it (Diff) & \it 0.1064 & \it 0.1379 & \it 0.0222 & \it 0.1087 & \it 0.1063 & \it 0.0963 \\
        \midrule
        & Likelihood & 0.9983 & 0.9949 & 0.9971 & 0.9960 & 0.9945 & 0.9962 \\
        & Entropy & 0.2511 & 0.3033 & 0.2190 & 0.2252 & 0.2625 & 0.2522 \\
        & LogRank & 0.9991 & 0.9972 & 0.9984 & 0.9977 & 0.9969 & 0.9978 \\
        & LRR & 0.9961 & 0.9917 & 0.9914 & 0.9887 & 0.9837 & 0.9903 \\
        & NPR & 0.9985 & 0.9953 & 0.9930 & 0.9836 & 0.9781 & 0.9897 \\
        \cdashline{2-8}
        Writing & DetectGPT & 0.9932 & 0.9850 & 0.9842 & 0.9656 & 0.9447 & 0.9745 \\
        Prompts & Fast-DetectGPT & 0.9997 & 0.9999 & 0.9992 & 0.9991 & 0.9984 & 0.9992 \\
        & \it (Diff) & \it 0.0065 & \it 0.0149 & \it 0.0150 & \it 0.0335 & \it 0.0537 & \it 0.0247 \\
        \cdashline{2-8}
        & DetectGPT & 0.9385 & 0.9451 & 0.9842 & 0.9535 & 0.9398 & 0.9522 \\
        & Fast-DetectGPT & 0.9995 & 0.9959 & 0.9997 & 0.9983 & 0.9987 & 0.9984 \\
        & \it (Diff) & \it 0.0610 & \it 0.0508 & \it 0.0155 & \it 0.0448 & \it 0.0588 & \it 0.0462 \\
        \bottomrule
    \end{tabular}
    \caption{Temperature decoding. Zero-shot detection accuracy (in AUROC), where Fast-DetectGPT consistently outperforms DetectGPT. ``(fixed)'' denotes using fixed models (the black-box setting), where DetectGPT uses T5-3B/Neo-2.7 as the perturbation/scoring models and Fast-DetectGPT uses GPT-J/Neo-2.7 as the sampling/scoring models.
    ``{\it (Diff)}'' rows indicate the AUROC improvement upon DetectGPT baselines. ``*'' denotes the second-best AUROC. $\diamondsuit$ -- Methods call models a hundred times, thus consuming much higher computational resources.}
    \label{tab:temperature_results}
\end{table}

==> tables/topk_results.tex <==
\begin{table}[t]
    \centering\scriptsize
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\bf Dataset} & \multirow{2}{*}{\bf Method} & \multicolumn{6}{c}{\bf Source Model} \\
         &  & GPT-2 & OPT-2.7 & Neo-2.7 & GPT-J & NeoX & \bf Avg. \\    
        \midrule
        \multirow{10}{*}{XSum} 
        & Likelihood & 0.8813 & 0.8918 & 0.8873 & 0.8401 & 0.8114 & 0.8624 \\
        & Entropy & 0.5743 & 0.4843 & 0.5601 & 0.5588 & 0.5917 & 0.5538 \\
        & LogRank & 0.9122 & 0.9173 & 0.9227 & 0.8756 & 0.8454 & 0.8946 \\
        & LRR & 0.9432 & 0.9254 & 0.9452 & 0.9045 & 0.8683 & 0.9173 \\
        & NPR & 0.9870 & 0.9801 & 0.9938 & 0.9606 & 0.9416 & 0.9726 \\
        \cdashline{2-8}
        & DetectGPT & 0.9869 & 0.9707 & 0.9919 & 0.9619 & 0.9424 & 0.9708 \\
        & Fast-DetectGPT & 0.9954 & 0.9867 & 0.9938 & 0.9826 & 0.9773 & 0.9871 \\
        & \it (Diff) & \it 0.0085 & \it 0.0160 & \it 0.0018 & \it 0.0207 & \it 0.0349 & \it 0.0164 \\
        \cdashline{2-8}
        & DetectGPT & 0.9143 & 0.9026 & 0.9919 & 0.8846 & 0.8854 & 0.9158 \\
        & Fast-DetectGPT & 0.9805 & 0.9613 & 0.9979 & 0.9499 & 0.9311 & 0.9642 \\
        & \it (Diff) & \it 0.0662 & \it 0.0587 & \it 0.0060 & \it 0.0654 & \it 0.0457 & \it 0.0484 \\
        \midrule
        \multirow{10}{*}{SQuAD}
        & Likelihood & 0.9393 & 0.9072 & 0.8926 & 0.8351 & 0.7317 & 0.8612 \\
        & Entropy & 0.5520 & 0.5203 & 0.5457 & 0.5441 & 0.5992 & 0.5523 \\
        & LogRank & 0.9692 & 0.9423 & 0.9385 & 0.8842 & 0.7895 & 0.9047 \\
        & LRR & 0.9898 & 0.9782 & 0.9815 & 0.9450 & 0.8886 & 0.9566 \\
        & NPR & 0.9962 & 0.9900 & 0.9877 & 0.9251 & 0.8260 & 0.9450 \\
        \cdashline{2-8}
        & DetectGPT & 0.9928 & 0.9804 & 0.9709 & 0.8819 & 0.7977 & 0.9247 \\
        & Fast-DetectGPT & 0.9986 & 0.9973 & 0.9980 & 0.9928 & 0.9706 & 0.9914 \\
        & \it (Diff) & \it 0.0057 & \it 0.0169 & \it 0.0271 & \it 0.1109 & \it 0.1729 & \it 0.0667 \\
        \cdashline{2-8}
        & DetectGPT & 0.7815 & 0.7630 & 0.9709 & 0.8128 & 0.7729 & 0.8202 \\
        & Fast-DetectGPT & 0.9893 & 0.9840 & 0.9997 & 0.9709 & 0.9509 & 0.9790 \\
        & \it (Diff) & \it 0.2078 & \it 0.2210 & \it 0.0288 & \it 0.1581 & \it 0.1780 & \it 0.1587 \\
        \midrule
        & Likelihood & 0.9777 & 0.9555 & 0.9677 & 0.9566 & 0.9463 & 0.9608 \\
        & Entropy & 0.3601 & 0.4149 & 0.3183 & 0.3529 & 0.3696 & 0.3632 \\
        & LogRank & 0.9867 & 0.9719 & 0.9807 & 0.9735 & 0.9656 & 0.9757 \\
        & LRR & 0.9901 & 0.9835 & 0.9858 & 0.9834 & 0.9709 & 0.9827 \\
        & NPR & 0.9988 & 0.9955 & 0.9971 & 0.9888 & 0.9759 & 0.9912 \\
        \cdashline{2-8}
        Writing & DetectGPT & 0.9965 & 0.9868 & 0.9920 & 0.9710 & 0.9521 & 0.9797 \\
        Prompts & Fast-DetectGPT & 0.9978 & 0.9973 & 0.9990 & 0.9987 & 0.9957 & 0.9977 \\
        & \it (Diff) & \it 0.0012 & \it 0.0105 & \it 0.0070 & \it 0.0277 & \it 0.0436 & \it 0.0180 \\
        \cdashline{2-8}
        & DetectGPT & 0.9115 & 0.8906 & 0.9920 & 0.9052 & 0.8914 & 0.9181 \\
        & Fast-DetectGPT & 0.9947 & 0.9616 & 0.9998 & 0.9901 & 0.9860 & 0.9864 \\
        & \it (Diff) & \it 0.0832 & \it 0.0710 & \it 0.0079 & \it 0.0849 & \it 0.0946 & \it 0.0683 \\
        \bottomrule
    \end{tabular}
    \caption{Top-k decoding. Zero-shot detection accuracy (in AUROC), where Fast-DetectGPT consistently outperforms DetectGPT. ``(fixed)'' denotes using fixed models (the black-box setting), where DetectGPT uses T5-3B/Neo-2.7 as the perturbation/scoring models and Fast-DetectGPT uses GPT-J/Neo-2.7 as the sampling/scoring models.
    ``{\it (Diff)}'' rows indicate the AUROC improvement upon DetectGPT baselines. ``*'' denotes the second-best AUROC. $\diamondsuit$ -- Methods call models a hundred times, thus consuming much higher computational resources.}
    \label{tab:topk_results}
\end{table}

==> tables/topp_results.tex <==
\begin{table}[t]
    \centering\scriptsize
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\bf Dataset} & \multirow{2}{*}{\bf Method} & \multicolumn{6}{c}{\bf Source Model} \\
         &  & GPT-2 & OPT-2.7 & Neo-2.7 & GPT-J & NeoX & \bf Avg. \\    
        \midrule
        \multirow{10}{*}{XSum} 
        & Likelihood & 0.9234 & 0.9308 & 0.9310 & 0.9042 & 0.8733 & 0.9126 \\
        & Entropy & 0.5541 & 0.4665 & 0.5303 & 0.5310 & 0.5614 & 0.5287 \\
        & LogRank & 0.9414 & 0.9422 & 0.9502 & 0.9220 & 0.8906 & 0.9293 \\
        & LRR & 0.9509 & 0.9252 & 0.9478 & 0.9203 & 0.8672 & 0.9223 \\
        & NPR & 0.9909 & 0.9841 & 0.9982 & 0.9730 & 0.9486 & 0.9789 \\
        \cdashline{2-8}
        & DetectGPT & 0.9875 & 0.9793 & 0.9961 & 0.9762 & 0.9500 & 0.9778 \\
        & Fast-DetectGPT & 0.9994 & 0.9965 & 0.9988 & 0.9970 & 0.9958 & 0.9975 \\
        & \it (Diff) & \it 0.0119 & \it 0.0172 & \it 0.0028 & \it 0.0208 & \it 0.0458 & \it 0.0197 \\
        \cdashline{2-8}
        & DetectGPT & 0.9399 & 0.9438 & 0.9961 & 0.9367 & 0.9214 & 0.9476 \\
        & Fast-DetectGPT & 0.9953 & 0.9861 & 0.9997 & 0.9856 & 0.9779 & 0.9889 \\
        & \it (Diff) & \it 0.0554 & \it 0.0423 & \it 0.0036 & \it 0.0489 & \it 0.0565 & \it 0.0413 \\
        \midrule
        \multirow{10}{*}{SQuAD}
        & Likelihood & 0.9610 & 0.9440 & 0.9214 & 0.8838 & 0.8122 & 0.9045 \\
        & Entropy & 0.5369 & 0.4736 & 0.5390 & 0.5277 & 0.5593 & 0.5273 \\
        & LogRank & 0.9792 & 0.9657 & 0.9535 & 0.9156 & 0.8482 & 0.9324 \\
        & LRR & 0.9865 & 0.9810 & 0.9810 & 0.9507 & 0.9009 & 0.9600 \\
        & NPR & 0.9955 & 0.9934 & 0.9897 & 0.9335 & 0.8436 & 0.9511 \\
        \cdashline{2-8}
        & DetectGPT & 0.9940 & 0.9838 & 0.9781 & 0.9054 & 0.8182 & 0.9359 \\
        & Fast-DetectGPT & 1.0000 & 0.9997 & 0.9998 & 0.9981 & 0.9903 & 0.9976 \\
        & \it (Diff) & \it 0.0060 & \it 0.0159 & \it 0.0218 & \it 0.0927 & \it 0.1722 & \it 0.0617 \\
        \cdashline{2-8}
        & DetectGPT & 0.8066 & 0.7857 & 0.9781 & 0.8462 & 0.8365 & 0.8506 \\
        & Fast-DetectGPT & 0.9984 & 0.9950 & 1.0000 & 0.9933 & 0.9845 & 0.9942 \\
        & \it (Diff) & \it 0.1918 & \it 0.2093 & \it 0.0219 & \it 0.1471 & \it 0.1480 & \it 0.1436 \\
        \midrule
        & Likelihood & 0.9889 & 0.9736 & 0.9806 & 0.9764 & 0.9711 & 0.9781 \\
        & Entropy & 0.3236 & 0.3789 & 0.2798 & 0.3212 & 0.3238 & 0.3255 \\
        & LogRank & 0.9931 & 0.9827 & 0.9870 & 0.9853 & 0.9785 & 0.9853 \\
        & LRR & 0.9906 & 0.9854 & 0.9857 & 0.9839 & 0.9724 & 0.9836 \\
        & NPR & 0.9984 & 0.9964 & 0.9944 & 0.9855 & 0.9758 & 0.9901 \\
        \cdashline{2-8}
        Writing & DetectGPT & 0.9969 & 0.9898 & 0.9926 & 0.9714 & 0.9526 & 0.9807 \\
        Prompts & Fast-DetectGPT & 0.9997 & 0.9999 & 0.9998 & 0.9998 & 0.9981 & 0.9994 \\
        & \it (Diff) & \it 0.0028 & \it 0.0102 & \it 0.0071 & \it 0.0284 & \it 0.0455 & \it 0.0188 \\
        \cdashline{2-8}
        & DetectGPT & 0.9297 & 0.9177 & 0.9926 & 0.9299 & 0.9187 & 0.9377 \\
        & Fast-DetectGPT & 0.9982 & 0.9825 & 0.9999 & 0.9974 & 0.9945 & 0.9945 \\
        & \it (Diff) & \it 0.0685 & \it 0.0648 & \it 0.0073 & \it 0.0676 & \it 0.0758 & \it 0.0568 \\
        \bottomrule
    \end{tabular}
    \caption{Top-p decoding. Zero-shot detection accuracy (in AUROC), where Fast-DetectGPT consistently outperforms DetectGPT. ``(fixed)'' denotes using fixed models (the black-box setting), where DetectGPT uses T5-3B/Neo-2.7 as the perturbation/scoring models and Fast-DetectGPT uses GPT-J/Neo-2.7 as the sampling/scoring models.
    ``{\it (Diff)}'' rows indicate the AUROC improvement upon DetectGPT baselines. ``*'' denotes the second-best AUROC. $\diamondsuit$ -- Methods call models a hundred times, thus consuming much higher computational resources.}
    \label{tab:topp_results}
\end{table}
